Online and Offline Robust Multivariate Linear Regression

We consider the robust estimation of the parameters of multivariate Gaussian linear regression models. To this aim we consider robust version of the usual (Mahalanobis) least-square criterion, with or without Ridge regularization. We introduce two methods each considered contrast: (i) online stochastic gradient descent algorithms and their averaged versions and (ii) offline fix-point algorithms. Under weak assumptions, we prove the asymptotic normality of the resulting estimates. Because the variance matrix of the noise is usually unknown, we propose to plug a robust estimate of it in the Mahalanobis-based stochastic gradient descent algorithms. We show, on synthetic data, the dramatic gain in terms of robustness of the proposed estimates as compared to the classical least-square ones. Well also show the computational efficiency of the online versions of the proposed algorithms. All the proposed algorithms are implemented in the R package RobRegression available on CRAN.

==> TablesV2/AUC-n1000-fake-p5-q20-k1-sd1-seed1-df1-WLS+Ridge.tex <==
\begin{tabular}{r|rrrrrr} 
& \multicolumn{2}{c}{ Naive } & \multicolumn{2}{c}{ Offline } & \multicolumn{2}{c}{ Online } \\ 
\hline 
2  &0.67  & ( 0.087 ) & 0.67  & ( 0.091 ) & 0.67  & ( 0.09 ) \\ 
3  &0.68  & ( 0.078 ) & 0.67  & ( 0.083 ) & 0.67  & ( 0.083 ) \\ 
5  &0.67  & ( 0.064 ) & 0.67  & ( 0.065 ) & 0.67  & ( 0.065 ) \\ 
9  &0.67  & ( 0.042 ) & 0.66  & ( 0.045 ) & 0.66  & ( 0.045 ) \\ 
16  &0.67  & ( 0.03 ) & 0.66  & ( 0.033 ) & 0.66  & ( 0.033 ) \\ 
28  &0.66  & ( 0.024 ) & 0.66  & ( 0.027 ) & 0.66  & ( 0.027 ) \\ 
50  &0.64  & ( 0.02 ) & 0.65  & ( 0.019 ) & 0.65  & ( 0.019 ) \\ 
\end{tabular} 
 


==> TablesV2/AUC-n1000-fake-p5-q20-k1-sd1-seed1-df1-WLS.tex <==
\begin{tabular}{r|rrrrrr} 
& \multicolumn{2}{c}{ Naive } & \multicolumn{2}{c}{ Offline } & \multicolumn{2}{c}{ Online } \\ 
\hline 
2  &0.67  & ( 0.089 ) & 0.67  & ( 0.091 ) & 0.67  & ( 0.09 ) \\ 
3  &0.67  & ( 0.081 ) & 0.67  & ( 0.083 ) & 0.67  & ( 0.083 ) \\ 
5  &0.66  & ( 0.065 ) & 0.67  & ( 0.064 ) & 0.67  & ( 0.065 ) \\ 
9  &0.66  & ( 0.044 ) & 0.67  & ( 0.046 ) & 0.67  & ( 0.046 ) \\ 
16  &0.64  & ( 0.032 ) & 0.66  & ( 0.033 ) & 0.66  & ( 0.033 ) \\ 
28  &0.63  & ( 0.03 ) & 0.66  & ( 0.028 ) & 0.66  & ( 0.028 ) \\ 
50  &0.6  & ( 0.025 ) & 0.65  & ( 0.019 ) & 0.65  & ( 0.019 ) \\ 
\end{tabular} 
 


==> TablesV2/MSEbeta-n1000-fake-p5-q20-k1-sd1-seed1-df1-WLS+Ridge.tex <==
\begin{tabular}{r|rrrrrr} 
& \multicolumn{2}{c}{ Naive } & \multicolumn{2}{c}{ Offline } & \multicolumn{2}{c}{ Online } \\ 
\hline 
0  &0.0018  & ( 0.00058 ) & 0.0018  & ( 6e-04 ) & 0.0028  & ( 0.00097 ) \\ 
2  &0.076  & ( 0.2 ) & 0.0018  & ( 0.00074 ) & 0.0031  & ( 0.0016 ) \\ 
3  &0.048  & ( 0.13 ) & 0.0019  & ( 0.00079 ) & 0.003  & ( 0.0014 ) \\ 
5  &0.091  & ( 0.19 ) & 0.0026  & ( 0.0077 ) & 0.0037  & ( 0.0074 ) \\ 
9  &0.28  & ( 0.31 ) & 0.018  & ( 0.11 ) & 0.028  & ( 0.18 ) \\ 
16  &0.46  & ( 0.27 ) & 0.0031  & ( 0.0048 ) & 0.0038  & ( 0.0038 ) \\ 
28  &0.65  & ( 0.17 ) & 0.019  & ( 0.11 ) & 0.03  & ( 0.18 ) \\ 
50  &0.76  & ( 0.026 ) & 0.0047  & ( 0.0087 ) & 0.0057  & ( 0.008 ) \\ 
\end{tabular} 
 


==> TablesV2/MSEbeta-n1000-fake-p5-q20-k1-sd1-seed1-df1-WLS.tex <==
\begin{tabular}{r|rrrrrr} 
& \multicolumn{2}{c}{ Naive } & \multicolumn{2}{c}{ Offline } & \multicolumn{2}{c}{ Online } \\ 
\hline 
0  &0.0018  & ( 0.00058 ) & 0.0018  & ( 0.00061 ) & 0.003  & ( 0.0011 ) \\ 
2  &0.14  & ( 0.6 ) & 0.0018  & ( 0.00053 ) & 0.0031  & ( 0.0014 ) \\ 
3  &0.06  & ( 0.38 ) & 0.0018  & ( 0.00055 ) & 0.0032  & ( 0.0017 ) \\ 
5  &0.16  & ( 0.81 ) & 0.0018  & ( 5e-04 ) & 0.0029  & ( 0.0011 ) \\ 
9  &14  & ( 140 ) & 0.0018  & ( 0.00054 ) & 0.0032  & ( 0.0014 ) \\ 
16  &1.6  & ( 7.9 ) & 0.0018  & ( 0.00053 ) & 0.0029  & ( 0.0011 ) \\ 
28  &5.2  & ( 30 ) & 0.0018  & ( 0.00052 ) & 0.0031  & ( 0.0014 ) \\ 
50  &3.3  & ( 17 ) & 0.0017  & ( 0.00039 ) & 0.0029  & ( 0.00096 ) \\ 
\end{tabular} 
 


==> TablesV2/MSEbeta-prop28-fake-p5-q20-k1-sd1-seed1-df1-WLS+Ridge.tex <==
\begin{tabular}{r|rrrrrr} 
& \multicolumn{2}{c}{ Naive } & \multicolumn{2}{c}{ Offline } & \multicolumn{2}{c}{ Online } \\ 
\hline 
100  &0.45  & ( 0.3 ) & 0.054  & ( 0.15 ) & 0.46  & ( 0.73 ) \\ 
1000  &0.65  & ( 0.17 ) & 0.019  & ( 0.11 ) & 0.03  & ( 0.18 ) \\ 
10000  &0.77  & ( 0.019 ) & 0.013  & ( 0.082 ) & 0.033  & ( 0.28 ) \\ 
\end{tabular} 
 


==> TablesV2/MSEbeta-prop28-fake-p5-q20-k1-sd1-seed1-df1-WLS.tex <==
\begin{tabular}{r|rrrrrr} 
& \multicolumn{2}{c}{ Naive } & \multicolumn{2}{c}{ Offline } & \multicolumn{2}{c}{ Online } \\ 
\hline 
100  &85  & ( 660 ) & 0.019  & ( 0.0058 ) & 2.3  & ( 4.4 ) \\ 
1000  &5.2  & ( 30 ) & 0.0018  & ( 0.00052 ) & 0.0031  & ( 0.0014 ) \\ 
10000  &19  & ( 130 ) & 0.00017  & ( 4.1e-05 ) & 0.00033  & ( 0.00021 ) \\ 
\end{tabular} 
 


==> TablesV2/MSEbeta-prop5-fake-p5-q20-k1-sd1-seed1-df1-WLS+Ridge.tex <==
\begin{tabular}{r|rrrrrr} 
& \multicolumn{2}{c}{ Naive } & \multicolumn{2}{c}{ Offline } & \multicolumn{2}{c}{ Online } \\ 
\hline 
100  &0.063  & ( 0.15 ) & 0.019  & ( 0.0065 ) & 0.29  & ( 0.13 ) \\ 
1000  &0.091  & ( 0.19 ) & 0.0026  & ( 0.0077 ) & 0.0037  & ( 0.0074 ) \\ 
10000  &0.22  & ( 0.26 ) & 0.00065  & ( 0.0039 ) & 0.00075  & ( 0.0037 ) \\ 
\end{tabular} 
 


==> TablesV2/MSEbeta-prop5-fake-p5-q20-k1-sd1-seed1-df1-WLS.tex <==
\begin{tabular}{r|rrrrrr} 
& \multicolumn{2}{c}{ Naive } & \multicolumn{2}{c}{ Offline } & \multicolumn{2}{c}{ Online } \\ 
\hline 
100  &0.17  & ( 0.85 ) & 0.019  & ( 0.0063 ) & 1.5  & ( 3.1 ) \\ 
1000  &0.16  & ( 0.81 ) & 0.0018  & ( 5e-04 ) & 0.0029  & ( 0.0011 ) \\ 
10000  &0.22  & ( 1.1 ) & 0.00017  & ( 5.5e-05 ) & 0.00032  & ( 0.00018 ) \\ 
\end{tabular} 
 


==> TablesV2/MSEbetacompOW-Ridge-n1000-fake-p5-q20-k1-sd1-seed1-df1-Off.tex <==
\begin{tabular}{r|rrrr} 
& \multicolumn{2}{c}{ OLS } & \multicolumn{2}{c}{ WLS } \\ 
\hline 
0  &0.0019  & ( 0.00066 ) & 0.0018  & ( 6e-04 ) \\ 
2  &0.002  & ( 0.00091 ) & 0.0018  & ( 0.00074 ) \\ 
3  &0.0019  & ( 0.00058 ) & 0.0019  & ( 0.00079 ) \\ 
5  &0.0028  & ( 0.0096 ) & 0.0026  & ( 0.0077 ) \\ 
9  &0.018  & ( 0.11 ) & 0.018  & ( 0.11 ) \\ 
16  &0.0027  & ( 0.004 ) & 0.0031  & ( 0.0048 ) \\ 
28  &0.019  & ( 0.11 ) & 0.019  & ( 0.11 ) \\ 
50  &0.0048  & ( 0.009 ) & 0.0047  & ( 0.0087 ) \\ 
\end{tabular} 
 


==> TablesV2/MSEbetacompOW-Ridge-n1000-fake-p5-q20-k1-sd1-seed1-df1-On.tex <==
\begin{tabular}{r|rrrr} 
& \multicolumn{2}{c}{ OLS } & \multicolumn{2}{c}{ WLS } \\ 
\hline 
0  &0.0059  & ( 0.002 ) & 0.0028  & ( 0.00097 ) \\ 
2  &0.0062  & ( 0.0025 ) & 0.0031  & ( 0.0016 ) \\ 
3  &0.0063  & ( 0.0029 ) & 0.003  & ( 0.0014 ) \\ 
5  &0.011  & ( 0.044 ) & 0.0037  & ( 0.0074 ) \\ 
9  &0.022  & ( 0.1 ) & 0.028  & ( 0.18 ) \\ 
16  &0.011  & ( 0.032 ) & 0.0038  & ( 0.0038 ) \\ 
28  &0.022  & ( 0.098 ) & 0.03  & ( 0.18 ) \\ 
50  &0.01  & ( 0.0081 ) & 0.0057  & ( 0.008 ) \\ 
\end{tabular} 
 


==> TablesV2/MSEbetacompOW-n1000-fake-p5-q20-k1-sd1-seed1-df1-Off+Ridge.tex <==
\begin{tabular}{r|rrrr} 
& \multicolumn{2}{c}{ OLS } & \multicolumn{2}{c}{ WLS } \\ 
\hline 
0  &0.0019  & ( 0.00066 ) & 0.0018  & ( 6e-04 ) \\ 
2  &0.002  & ( 0.00091 ) & 0.0018  & ( 0.00074 ) \\ 
3  &0.0019  & ( 0.00058 ) & 0.0019  & ( 0.00079 ) \\ 
5  &0.0028  & ( 0.0096 ) & 0.0026  & ( 0.0077 ) \\ 
9  &0.018  & ( 0.11 ) & 0.018  & ( 0.11 ) \\ 
16  &0.0027  & ( 0.004 ) & 0.0031  & ( 0.0048 ) \\ 
28  &0.019  & ( 0.11 ) & 0.019  & ( 0.11 ) \\ 
50  &0.0048  & ( 0.009 ) & 0.0047  & ( 0.0087 ) \\ 
\end{tabular} 
 


==> TablesV2/MSEbetacompOW-n1000-fake-p5-q20-k1-sd1-seed1-df1-Off.tex <==
\begin{tabular}{r|rrrr} 
& \multicolumn{2}{c}{ OLS } & \multicolumn{2}{c}{ WLS } \\ 
\hline 
0  &0.0019  & ( 0.00066 ) & 0.0018  & ( 0.00061 ) \\ 
2  &0.0019  & ( 0.00053 ) & 0.0018  & ( 0.00053 ) \\ 
3  &0.0019  & ( 0.00055 ) & 0.0018  & ( 0.00055 ) \\ 
5  &0.0019  & ( 0.00053 ) & 0.0018  & ( 5e-04 ) \\ 
9  &0.0019  & ( 0.00052 ) & 0.0018  & ( 0.00054 ) \\ 
16  &0.0018  & ( 0.00051 ) & 0.0018  & ( 0.00053 ) \\ 
28  &0.0018  & ( 0.00046 ) & 0.0018  & ( 0.00052 ) \\ 
50  &0.0016  & ( 0.00035 ) & 0.0017  & ( 0.00039 ) \\ 
\end{tabular} 
 


==> TablesV2/MSEbetacompOW-n1000-fake-p5-q20-k1-sd1-seed1-df1-On+Ridge.tex <==
\begin{tabular}{r|rrrr} 
& \multicolumn{2}{c}{ OLS } & \multicolumn{2}{c}{ WLS } \\ 
\hline 
0  &0.0059  & ( 0.002 ) & 0.0028  & ( 0.00097 ) \\ 
2  &0.0062  & ( 0.0025 ) & 0.0031  & ( 0.0016 ) \\ 
3  &0.0063  & ( 0.0029 ) & 0.003  & ( 0.0014 ) \\ 
5  &0.011  & ( 0.044 ) & 0.0037  & ( 0.0074 ) \\ 
9  &0.022  & ( 0.1 ) & 0.028  & ( 0.18 ) \\ 
16  &0.011  & ( 0.032 ) & 0.0038  & ( 0.0038 ) \\ 
28  &0.022  & ( 0.098 ) & 0.03  & ( 0.18 ) \\ 
50  &0.01  & ( 0.0081 ) & 0.0057  & ( 0.008 ) \\ 
\end{tabular} 
 


==> TablesV2/MSEbetacompOW-n1000-fake-p5-q20-k1-sd1-seed1-df1-On.tex <==
\begin{tabular}{r|rrrr} 
& \multicolumn{2}{c}{ OLS } & \multicolumn{2}{c}{ WLS } \\ 
\hline 
0  &0.0067  & ( 0.0033 ) & 0.003  & ( 0.0011 ) \\ 
2  &0.0068  & ( 0.0034 ) & 0.0031  & ( 0.0014 ) \\ 
3  &0.0077  & ( 0.008 ) & 0.0032  & ( 0.0017 ) \\ 
5  &0.0073  & ( 0.0045 ) & 0.0029  & ( 0.0011 ) \\ 
9  &0.0071  & ( 0.0036 ) & 0.0032  & ( 0.0014 ) \\ 
16  &0.0074  & ( 0.0041 ) & 0.0029  & ( 0.0011 ) \\ 
28  &0.0075  & ( 0.0034 ) & 0.0031  & ( 0.0014 ) \\ 
50  &0.0079  & ( 0.0035 ) & 0.0029  & ( 0.00096 ) \\ 
\end{tabular} 
 


==> TablesV2/MSEsigma-n1000-fake-p5-q20-k1-sd1-seed1-df1-Ridge.tex <==
\begin{tabular}{r|rrrrrr} 
& \multicolumn{2}{c}{ Naive } & \multicolumn{2}{c}{ Offline } & \multicolumn{2}{c}{ Online } \\ 
\hline 
0  &0.0043  & ( 0.0026 ) & 0.0058  & ( 0.0038 ) & 0.006  & ( 0.0034 ) \\ 
2  &430000  & ( 2400000 ) & 0.0063  & ( 0.004 ) & 0.0066  & ( 0.004 ) \\ 
3  &370000  & ( 3600000 ) & 0.0067  & ( 0.0039 ) & 0.0084  & ( 0.013 ) \\ 
5  &4e+05  & ( 2400000 ) & 0.0093  & ( 0.0062 ) & 0.009  & ( 0.0057 ) \\ 
9  &3e+09  & ( 3e+10 ) & 0.017  & ( 0.01 ) & 0.016  & ( 0.0091 ) \\ 
16  &5e+07  & ( 2.8e+08 ) & 0.036  & ( 0.016 ) & 0.034  & ( 0.016 ) \\ 
28  &2e+10  & ( 2e+11 ) & 0.098  & ( 0.022 ) & 0.093  & ( 0.021 ) \\ 
50  &4.4e+08  & ( 4.1e+09 ) & 0.27  & ( 0.024 ) & 0.26  & ( 0.025 ) \\ 
\end{tabular} 
 


==> TablesV2/MSEsigma-n1000-fake-p5-q20-k1-sd1-seed1-df1-noRidge.tex <==
\begin{tabular}{r|rrrrrrrr} 
& \multicolumn{2}{c}{ Naive } & \multicolumn{2}{c}{ Offline } & \multicolumn{2}{c}{ Online } & \multicolumn{2}{c}{ RRRR } \\ 
\hline 
0  &0.0043  & ( 0.0026 ) & 0.0058  & ( 0.0035 ) & 0.0059  & ( 0.0034 ) & 0.031  & ( 0.011 ) \\ 
2  &430000  & ( 2400000 ) & 0.0064  & ( 0.0039 ) & 0.0066  & ( 0.0038 ) & 0.034  & ( 0.012 ) \\ 
3  &370000  & ( 3600000 ) & 0.0067  & ( 0.0043 ) & 0.0082  & ( 0.013 ) & 0.038  & ( 0.011 ) \\ 
5  &4e+05  & ( 2400000 ) & 0.0092  & ( 0.0058 ) & 0.009  & ( 0.006 ) & 0.041  & ( 0.013 ) \\ 
9  &3e+09  & ( 3e+10 ) & 0.016  & ( 0.0096 ) & 0.015  & ( 0.0091 ) & 0.055  & ( 0.015 ) \\ 
16  &5e+07  & ( 2.8e+08 ) & 0.037  & ( 0.016 ) & 0.034  & ( 0.016 ) & 0.08  & ( 0.019 ) \\ 
28  &2e+10  & ( 2e+11 ) & 0.098  & ( 0.022 ) & 0.092  & ( 0.022 ) & 0.14  & ( 0.02 ) \\ 
50  &4.4e+08  & ( 4.1e+09 ) & 0.27  & ( 0.024 ) & 0.26  & ( 0.025 ) & 0.28  & ( 0.026 ) \\ 
\end{tabular} 
 


==> TablesV2/PredIn-n1000-fake-p5-q20-k1-sd1-seed1-df1-OLS+Ridge.tex <==
\begin{tabular}{r|rrrrrr} 
& \multicolumn{2}{c}{ Naive } & \multicolumn{2}{c}{ Offline } & \multicolumn{2}{c}{ Online } \\ 
\hline 
0  &1.8  & ( 0.042 ) & 1.8  & ( 0.042 ) & 1.8  & ( 0.042 ) \\ 
2  &2.1  & ( 0.82 ) & 1.8  & ( 0.04 ) & 1.8  & ( 0.044 ) \\ 
3  &1.9  & ( 0.54 ) & 1.8  & ( 0.039 ) & 1.8  & ( 0.042 ) \\ 
5  &2  & ( 0.7 ) & 1.8  & ( 0.061 ) & 1.9  & ( 0.22 ) \\ 
9  &2.4  & ( 1 ) & 1.9  & ( 0.56 ) & 1.9  & ( 0.53 ) \\ 
16  &2.7  & ( 1.2 ) & 1.8  & ( 0.049 ) & 1.9  & ( 0.17 ) \\ 
28  &2.8  & ( 1.2 ) & 1.9  & ( 0.54 ) & 1.9  & ( 0.48 ) \\ 
50  &3.6  & ( 1.3 ) & 1.8  & ( 0.07 ) & 1.9  & ( 0.066 ) \\ 
\end{tabular} 
 


==> TablesV2/PredIn-n1000-fake-p5-q20-k1-sd1-seed1-df1-OLS.tex <==
\begin{tabular}{r|rrrrrrrr} 
& \multicolumn{2}{c}{ Naive } & \multicolumn{2}{c}{ Offline } & \multicolumn{2}{c}{ Online } & \multicolumn{2}{c}{ RRRR } \\ 
\hline 
0  &1.8  & ( 0.042 ) & 1.8  & ( 0.042 ) & 1.8  & ( 0.043 ) & 1.8  & ( 0.042 ) \\ 
2  &2.5  & ( 3 ) & 1.8  & ( 0.04 ) & 1.8  & ( 0.046 ) & 1.8  & ( 0.04 ) \\ 
3  &2.1  & ( 2.2 ) & 1.8  & ( 0.039 ) & 1.8  & ( 0.057 ) & 1.8  & ( 0.039 ) \\ 
5  &2.6  & ( 4.3 ) & 1.8  & ( 0.041 ) & 1.9  & ( 0.048 ) & 1.8  & ( 0.041 ) \\ 
9  &79  & ( 760 ) & 1.8  & ( 0.041 ) & 1.8  & ( 0.045 ) & 1.8  & ( 0.041 ) \\ 
16  &11  & ( 45 ) & 1.8  & ( 0.046 ) & 1.9  & ( 0.051 ) & 1.8  & ( 0.046 ) \\ 
28  &29  & ( 160 ) & 1.8  & ( 0.043 ) & 1.8  & ( 0.046 ) & 1.8  & ( 0.043 ) \\ 
50  &19  & ( 89 ) & 1.8  & ( 0.056 ) & 1.9  & ( 0.057 ) & 1.8  & ( 0.056 ) \\ 
\end{tabular} 
 


==> TablesV2/PredIn-n1000-fake-p5-q20-k1-sd1-seed1-df1-WLS+Ridge.tex <==
\begin{tabular}{r|rrrrrr} 
& \multicolumn{2}{c}{ Naive } & \multicolumn{2}{c}{ Offline } & \multicolumn{2}{c}{ Online } \\ 
\hline 
0  &1.8  & ( 0.042 ) & 1.8  & ( 0.042 ) & 1.8  & ( 0.042 ) \\ 
2  &2.2  & ( 1 ) & 1.8  & ( 0.039 ) & 1.8  & ( 0.041 ) \\ 
3  &2.1  & ( 0.7 ) & 1.8  & ( 0.039 ) & 1.8  & ( 0.039 ) \\ 
5  &2.3  & ( 1 ) & 1.8  & ( 0.055 ) & 1.8  & ( 0.054 ) \\ 
9  &3.3  & ( 1.6 ) & 1.9  & ( 0.56 ) & 2  & ( 1 ) \\ 
16  &4.2  & ( 1.4 ) & 1.8  & ( 0.051 ) & 1.8  & ( 0.05 ) \\ 
28  &5.2  & ( 0.9 ) & 1.9  & ( 0.54 ) & 2  & ( 0.9 ) \\ 
50  &5.8  & ( 0.21 ) & 1.8  & ( 0.07 ) & 1.8  & ( 0.065 ) \\ 
\end{tabular} 
 


==> TablesV2/PredIn-n1000-fake-p5-q20-k1-sd1-seed1-df1-WLS.tex <==
\begin{tabular}{r|rrrrrr} 
& \multicolumn{2}{c}{ Naive } & \multicolumn{2}{c}{ Offline } & \multicolumn{2}{c}{ Online } \\ 
\hline 
0  &1.8  & ( 0.042 ) & 1.8  & ( 0.042 ) & 1.8  & ( 0.042 ) \\ 
2  &2.5  & ( 3 ) & 1.8  & ( 0.04 ) & 1.8  & ( 0.04 ) \\ 
3  &2.1  & ( 2.2 ) & 1.8  & ( 0.039 ) & 1.8  & ( 0.039 ) \\ 
5  &2.6  & ( 4.3 ) & 1.8  & ( 0.041 ) & 1.8  & ( 0.041 ) \\ 
9  &79  & ( 760 ) & 1.8  & ( 0.041 ) & 1.8  & ( 0.042 ) \\ 
16  &11  & ( 45 ) & 1.8  & ( 0.046 ) & 1.8  & ( 0.047 ) \\ 
28  &29  & ( 160 ) & 1.8  & ( 0.043 ) & 1.8  & ( 0.043 ) \\ 
50  &19  & ( 89 ) & 1.8  & ( 0.056 ) & 1.8  & ( 0.056 ) \\ 
\end{tabular} 
 

